Spade: An Expression-Based HDL With Pipelines

Spade is a new open source hardware description language (HDL) designed to increase developer productivity without sacrificing the low-level control offered by HDLs. It is a standalone language which takes inspiration from modern software languages, and adds useful abstractions for common hardware constructs. It also comes with a convenient set of tooling, such as a helpful compiler, a build system with dependency management, tools for debugging, and editor integration.

==> common_tex/mintedsetup.tex <==
\setminted[rust]{fontsize=\small, autogobble}
\setminted[llvm]{fontsize=\small, autogobble}
\setminted[c++]{fontsize=\small, autogobble}


==> common_tex/pseudosetup.tex <==
  \catcode`\!=\active
  \catcode`@=\active
  \def!#1!{\textcolor{blue}{#1}}
  \def@#1@{\textit{#1}}

